Object Detectors in the Open Environment: Challenges, Solutions, and Outlook

With the emergence of foundation models, deep learning-based object detectors have shown practical usability in closed set scenarios. However, for real-world tasks, object detectors often operate in open environments, where crucial factors (e.g., data distribution, objective) that influence model learning are often changing. The dynamic and intricate nature of the open environment poses novel and formidable challenges to object detectors. Unfortunately, current research on object detectors in open environments lacks a comprehensive analysis of their distinctive characteristics, challenges, and corresponding solutions, which hinders their secure deployment in critical real-world scenarios. This paper aims to bridge this gap by conducting a comprehensive review and analysis of object detectors in open environments. We initially identified limitations of key structural components within the existing detection pipeline and propose the open environment object detector challenge framework that includes four quadrants (i.e., out-of-domain, out-of-category, robust learning, and incremental learning) based on the dimensions of the data / target changes. For each quadrant of challenges in the proposed framework, we present a detailed description and systematic analysis of the overarching goals and core difficulties, systematically review the corresponding solutions, and benchmark their performance over multiple widely adopted datasets. In addition, we engage in a discussion of open problems and potential avenues for future research. This paper aims to provide a fresh, comprehensive, and systematic understanding of the challenges and solutions associated with open-environment object detectors, thus catalyzing the development of more solid applications in real-world scenarios. A project related to this survey can be found at https://github.com/LiangSiyuan21/OEOD_Survey.

==> bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in]{author/siyuan.jpg}}]{Siyuan Liang} is a Research Fellow at the School of Computing, National University of Singapore, specializing in adversarial machine learning and computer vision. She obtained her Ph.D. in Cyberspace Security from the University of the Chinese Academy of Sciences and a Bachelor's degree in Software Engineering from Sichuan University. Her work primarily focuses on developing robust AI models to enhance computer vision security.
\end{IEEEbiography}

\vspace{-10 mm}

\begin{IEEEbiography}[{\includegraphics[width=1in]{author/wangwei.jpg}}]{Wei Wang}
     is currently a post-doctoral candidate at the School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen university, Shenzhen, China. He received the Ph.D. degree at the School of Software Technology, Dalian University of Technology, Dalian, China, in 2022. He received the M.S. degree at the School of Computer Science and Technology from the Anhui University, Hefei, China, in 2018. He received the B.S. degree at the School of Science from the Anhui Agricultural University, Hefei, China, in 2015. His major research interests include  transfer learning, zero-shot learning, deep learning, etc.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in]{author/ruoyu.jpg}}]{Ruoyu Chen}
    is currently working toward the Ph.D. degree in the School of Cyber Security, University of Chinese Academy of Sciences, China. He received his B.E. degree in measurement \& control technology and instrument from Northeastern University, China in 2021. He has published multiple top journal and conference papers, such as ICLR. He has served as a reviewer for several top journals and conferences such as T-PAMI, ECCV, CVPR, ICML, ICCV, ICLR, and NeurIPS. His research interests mainly include computer vision, object detection, and interpretable AI.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in]{author/xiaochun.jpeg}}]{Xiaochun Cao}(Senior Member, IEEE)
    is a Professor and Dean of School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen University. He received the B.E. and M.E. degrees both in computer science from Beihang University (BUAA), China, and the Ph.D. degree in computer science from the University of Central Florida, USA, with his dissertation nominated for the university level Outstanding Dissertation Award. After graduation, he spent about three years at ObjectVideo Inc. as a Research Scientist. From 2008 to 2012, he was a professor at Tianjin University. Before joining SYSU, he was a professor at Institute of Information Engineering, Chinese Academy of Sciences. He has authored and coauthored over 200 journal and conference papers. In 2004 and 2010, he was the recipients of the Piero Zamperoni best student paper award at the International Conference on Pattern Recognition. He is on the editorial boards of IEEE \textsc{Transactions on Pattern Analysis and Machine Intelligence} and IEEE \textsc{Transactions on Image Processing}, and was on the editorial boards of IEEE \textsc{Transactions on Circuits and Systems for Video Technology} and IEEE \textsc{Transactions on Multimedia}.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in]{author/boxi.jpg}}]{Boxi Wun}
     received the B.S. degree in Computer Science from Zhejiang University, China, in 2016 and the Ph.D. degree in Computer Science from Zhejiang University, in 2022. He is an assistant professor in the School of Software Technology, Zhejiang University, China. His research interests include machine learning, generative model, and computer vision..
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in]{author/xiaochun.jpeg}}]{Xiaochun Cao}(Senior Member, IEEE)
    is a Professor and Dean of School of Cyber Science and Technology, Shenzhen Campus of Sun Yat-sen University. He received the B.E. and M.E. degrees both in computer science from Beihang University (BUAA), China, and the Ph.D. degree in computer science from the University of Central Florida, USA, with his dissertation nominated for the university level Outstanding Dissertation Award. After graduation, he spent about three years at ObjectVideo Inc. as a Research Scientist. From 2008 to 2012, he was a professor at Tianjin University. Before joining SYSU, he was a professor at Institute of Information Engineering, Chinese Academy of Sciences. He has authored and coauthored over 200 journal and conference papers. In 2004 and 2010, he was the recipients of the Piero Zamperoni best student paper award at the International Conference on Pattern Recognition. He is on the editorial boards of IEEE \textsc{Transactions on Pattern Analysis and Machine Intelligence} and IEEE \textsc{Transactions on Image Processing}, and was on the editorial boards of IEEE \textsc{Transactions on Circuits and Systems for Video Technology} and IEEE \textsc{Transactions on Multimedia}.
\end{IEEEbiography}

==> checklist.tex <==
\section*{Checklist}
\begin{itemize}
    \item [1]For all authors...
    \begin{itemize}
        \item [(a)]Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
        {\color{blue}{[YES]}} The main experiments and analysis are in Section~\ref{sec:big_experiment}, where our abstract and introduction mainly focus on.
        
        \item[(b)]Have you read the ethics review guidelines and ensured that your paper conforms to them?
        {\color{blue}{[YES]}}
        
        \item[(c)]Did you discuss any potential negative societal impacts of your work?
        {\color{orange}{[NO]}} We do not see any potential negative societal impacts of our work.
         
        \item[(d)]Did you describe the limitations of your work?
        {\color{blue}{[YES]}} In Section~\ref{sec:limit} of Supplementary Material, we describe the limitations of your work in detail.
    \end{itemize}
    
    \item[2]If you are including theoretical results..
    \begin{itemize}
        \item[(a)] Did you state the full set of assumptions of all theoretical results?
        {\color{gray}{[N/A]}}
        
        \item[(b)]Did you include complete proofs of all theoretical results?
        {\color{gray}{[N/A]}}
    \end{itemize}
    
    \item[3]If you ran experiments...
    \begin{itemize}
        \item [(a)]Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? 
        {\color{blue}{[YES]}} We provided detailed code, document, open resources link , instructions and website for benchmark, all of these can be found on our website mentioned in Appendix~\ref{sec:maintenance}.
        
        \item[(b)]Did you specify all the training details (e.g., data splits, hyper-parameters, how they were chosen)?
        {\color{blue}{[YES]}} We specify all important experiments details in Appendix~\ref{sec:exp_setup}. The full details are shown with our code.
        
        \item[(c)]Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
        {\color{orange}{[NO]}}
        
        \item[(d)]Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
        {\color{blue}{[YES]}} We provides the GPU type in Section~\ref{sec:reproducibility} of Supplementary Material.
    \end{itemize}
    
    \item[4]If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
    \begin{itemize}
        \item [(a)]If your work uses existing assets, did you cite the creators?
        {\color{blue}{[YES]}} We use 5 kinds of different noise datasets, and we cite them in Section~\ref{sec:natural_noise} of Supplementary Material.
        
        \item[(b)]Did you mention the license of the assets?
        {\color{blue}{[YES]}} We mention it in Section~\ref{sec:licenses} of Supplementary Material.
        
        \item[(c)]Did you include any new assets either in the supplemental material or as a URL?
        {\color{blue}{[YES]}} We provided our code pre-trained model. All URLs about this benchmark can be found on our website.
        
        \item[(d)]Did you discuss whether and how consent was obtained from people whose data you're using/curating?
        {\color{gray}{[N/A]}}
    \end{itemize}
    
    \item[5]If you used crowdsourcing or conducted research with human subjects...
    \begin{itemize}
        \item[(a)]  Did you include the full text of instructions given to participants and screenshots, if applicable?
        {\color{gray}{[N/A]}}
        
        \item[(b)]Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
        {\color{gray}{[N/A]}}
        
        \item[(c)]Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
        {\color{gray}{[N/A]}}
    \end{itemize}
\end{itemize}

























==> tables/multi-step_incremental_object_detection.tex <==
\begin{table}[b]
\centering
\caption{Results of multi-step incremental comparisons on MS-COCO (2014).}
\label{multi-step incremental object detection}
\resizebox{\columnwidth}{!}{
\setlength{\tabcolsep}{4pt}
\small

% \newcolumntype{Y}{>{\centering\arraybackslash}p{\dimexpr.5\columnwidth/3}}
\newcolumntype{Z}{>{\centering\arraybackslash}p{\dimexpr.55\columnwidth/4}}

\begin{tabular}{lccZZZZ}
\toprule
\multirow{2}{*}{\multicolumn{1}{c}{Method}} & \multirow{2}{*}{Paper List} & \multirow{2}{*}{Main Method} & \multicolumn{4}{c}{4 groups} \\ \cmidrule(l){4-7} 
 &  &  & A & B & C & D \\ \midrule
ILOD~\cite{shmelkov2017incremental} & ICCV 2017 & regular & 49.2 & 30.2 & 23.2 & 20.9 \\
CIFRCN~\cite{hao2019end} & ICME 2019 & replay/regular & 58.1 & 31.8 & 26.0 & 22.9 \\
RT-Net~\cite{cui2023rt} & APIN 2022 & replay/model/regular & 58.5 & 33.8 & 28.9 & 24.9 \\
MVCD~\cite{yang2022multi} & PR 2022 & regular & 61.0 & 37.4 & 27.9 & 22.6 \\
ORE+~\cite{joseph2021towards} & CVPR 2021 & replay/model & 56.3 & 38.9 & 29.3 & 26.7 \\
OW-DETR+~\cite{gupta2022ow} & CVPR 2022 & model & 59.2 & 42.9 & 30.8 & 27.8 \\ \bottomrule 
\end{tabular}
}
\end{table}
